DocTer: Documentation Guided Fuzzing for Testing Deep Learning API Functions

Input constraints are useful for many software development tasks. For example, input constraints of a function enable the generation of valid inputs, i.e., inputs that follow these constraints, to test the function deeper. API functions of deep learning (DL) libraries have DL specific input constraints, which are described informally in the free form API documentation. Existing constraint extraction techniques are ineffective for extracting DL specific input constraints. To fill this gap, we design and implement a new technique, DocTer, to analyze API documentation to extract DL specific input constraints for DL API functions. DocTer features a novel algorithm that automatically constructs rules to extract API parameter constraints from syntactic patterns in the form of dependency parse trees of API descriptions. These rules are then applied to a large volume of API documents in popular DL libraries to extract their input parameter constraints. To demonstrate the effectiveness of the extracted constraints, DocTer uses the constraints to enable the automatic generation of valid and invalid inputs to test DL API functions. Our evaluation on three popular DL libraries (TensorFlow, PyTorch, and MXNet) shows that the precision of DocTer in extracting input constraints is 85.4%. DocTer detects 94 bugs from 174 API functions, including one previously unknown security vulnerability that is now documented in the CVE database, while a baseline technique without input constraints detects only 59 bugs. Most (63) of the 94 bugs are previously unknown, 54 of which have been fixed or confirmed by developers after we report them. In addition, DocTer detects 43 inconsistencies in documents, 39 of which are fixed or confirmed.

==> img/api_example.tex <==


\begin{figure}[t]
    \centering
    % \vspace{-5mm}
    \subfloat[API Document\label{fig:API_example}]{%
       \includegraphics[clip=true,trim=0mm 1.5mm 0mm 0mm,width=\linewidth]{img/PT-14_bug_doc_v2.pdf}}
       \vspace{-3mm}
       \\
       
    %   \subfloat[Exceptions Thrown with Invalid Input\label{fig:API_example_baseline}]{%
    %   \includegraphics[clip=true,trim=0mm 1.5mm 0mm 0mm,width=\linewidth]{img/PT-14_baseline.pdf}}
    %   \vspace{-3mm}
       
    \subfloat[Extracted constraints\label{fig:API_example_constraint}]{%
       %\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.49\linewidth]{img/PT-14_extracted_constraints_v2.pdf}}
       \includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.49\linewidth]{img/PT-14_extracted_constraints_v3.pdf}}
       %\hfill
    \subfloat[Bug-triggering input\label{fig:API_example_input}]{%
       \includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.49\linewidth]{img/PT-14_input_v2.pdf}}
       \vspace{-3mm}
       \\
    \subfloat[Bug fix in \footnotesize{\texttt{ GridSamplerKernel.cpp}}\label{fig:API_example_fix}]{%
       \includegraphics[clip=true,trim=0mm 4mm 0mm 0mm,width=\linewidth]{img/PT-14_fix.pdf}}
       
    \vspace{-3mm}
	\caption{PyTorch document   % API function 
	%\footnotesize{
	%\texttt{grid\_sample},
 helps our tool detect a bug that was fixed after we reported it to PyTorch 
 developers.
	%\lin{please remove the extra whitespace (around the borders) of the four PDF files}
	}
	%\vspace{-2mm}
	\label{fig:API_example_all}
	\vspace{-5mm}
\end{figure}

==> img/layer_api.tex <==

\begin{figure}[t]
    \centering
    %\subfloat[Function Layer API\label{fig:func_layer_api}]{%
     %  \includegraphics[clip=true,trim=0mm 1.5mm 0mm %0mm,width=\linewidth]{img/function_layer_API.pdf}}
     %  \vspace{-3mm}
     %  \\
    %\subfloat[Class Layer API\label{fig:class_layer_api}]{%
    \includegraphics[clip=true,trim=0mm 4mm 0mm 0mm,width=\linewidth]{img/class_layer_API.pdf}
       %}
    \vspace{-5mm}   
	\caption{Example of Testing Class Layer API} 
	%Examples of Two Types of Layer APIs}
	\label{fig:layer_api_all}
	\vspace{-5mm}
\end{figure}



==> tab/CI_vs_VI.tex <==


\begin{table}[t]
\centering
\caption{
Break down of \textbf{verified new / new / all} bugs found.
}
\vspace{-3mm}
\label{tab:bug_CI_VI}

%\resizebox{\linewidth}{!}{
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}llr@{ }r@{ }l@{ }r@{ }r@{ }rr@{ }r@{ }rr@{ }r@{ }r@{}}
\toprule
\textbf{Approach} & &
\multicolumn{3}{c}{\textbf{TensorFlow}} & \multicolumn{3}{c}{\textbf{PyTorch}} & \multicolumn{3}{c}{\textbf{MXNet}} & \multicolumn{3}{c}{\textbf{Total}} \\



\midrule
BL+CSTR & ~CI
& 14~/& 32~/& 53                              
& 14~/& 17~/& 19            
& 9~/& 10~/& 13        
& 37~/& 59~/& \baseConstrCIAll
\\
& ~VI     
& 21~/& 38~/& 59                                      
& 2~/&  2~/&  2                                    
& 8~/&  10~/& 13                                  
& 31~/& 50~/& \baseConstrVIAll
\\


\midrule

\tool& ~CI     
&  17~/& 35~/& 55                                
&  16~/&  18~/&  23                                    
&  8~/&  12~/&  15                                  
& 41~/& 65~/& \oursCIAll                          
\\
(BL+CSTR+BDY)& ~VI     
& 25~/& 39~/& 61                                     
& 3~/&  3~/&  3                                    
& 5~/&  8~/&  11                                 
& 33~/& 50~/& \oursVIAll   
\\


\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}



==> tab/comparison_traditional.tex <==
\begin{table*}[htbp]

\caption{Comparison with state-of-the-art~\gv approaches. The number of bugs that only ~\tool fixes is in parentheses \hilight{\bf (\uniqueall)}.
%\hung{this highlighting look strange to me, was it not clear with just parentheses?}. \lin{just here or the last row? 
%what is strange about it? we don't want to use bold because bold is used to indicate the best tool for each benchmark. Also, this highlights the number of bugs that are unique to us}
%\hung{Here and the last row, can we do under score and/or italic and parentheses?, It does not look good to me.}
The results are displayed as x/y, with x the number of correct patches %(identical or semantically equivalent to the developer's patch) 
%\lin{similarly say correct patches,  if you are worried about   people not know what it means, can repeat the definition here}
and y the number of plausible patches. 
*~indicates tools whose manual fix patterns are used by TBAR. 
$^\dagger$ indicates the number of patches that are identical to developer patches---the minimal number of correct patches.
The highest number of correct patches for each benchmark is in {\bf bold}. 
}
\vspace{-2mm}
\centering
\label{tab:comp_trad_approaches}
\adjustbox{max width=0.79\linewidth}{
\begin{tabular}{clccccccr}

\toprule
                                                                                                  \multirow{3}{*}[-0.5em]{\textbf{FL}} & 
                                                                                                  \multirow{3}{*}[-0.5em]{\textbf{Tool}} & \multicolumn{2}{c}{\textbf{Java}}         & \multicolumn{2}{c}{\textbf{C}}         & \textbf{Python}   & \textbf{JavaScript} & \multirow{3}{*}[-0.5em]{\textbf{Total}} \\

\cmidrule(rr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}


                                                                                                  & \textbf{}          & \texttt{\textbf{Defects4J}} & \texttt{\textbf{QuixBugs}}    & \texttt{\textbf{Codeflaws}} & \texttt{\textbf{ManyBugs}} & \texttt{\textbf{QuixBugs}} & \texttt{\textbf{BugAID}}           & \textbf{}      \\
                                                                                                  & \textbf{}          & 395 bugs & 40 bugs    & 3,902 bugs & 69 bugs & 40 bugs & 12 bugs           & \textbf{}      \\

\midrule

\multirow{10}{*}[0.5em]{\rotatebox{-90}{\textbf{Standard}}}
																								  & \textbf{~1 (j)GenProg}~\cite{le2012genprog,martinez2016astor}   & 5/27               & 0/2                  & [255-369]/1423                  & 2/18              & -                 & -                   & [262-376]              \\
                                                                                                  & \textbf{~2 (j)Kali}~\cite{qi2015analysis,martinez2016astor}      & 1/22               & 1/2                  & -                  & 3/27              & -                 & -                   & 5              \\
                                                                                                  & \textbf{~3 RSRepair}~\cite{qi2013does}  & 0/44               & 2/4                  & -                  & 2/10              & -                 & -                   & 4              \\
                                                                                                  & \textbf{~4 Angelix}~\cite{mechtaev2016angelix}   & -                  & -                    & 318/591            & \textbf{18/39}             & -                 & -                   & 336            \\
                                                                                                  & \textbf{~5 Prophet}~\cite{long2018automatic}   & -                  & -                    & 301/839                  & 15/39             & -                 & -                   & 316             \\
                                                                                                  & \textbf{~6 SPR}~\cite{long2015staged}       & -                  & -                    & 283/783                  & 11/38             & -                 & -                   & 294             \\
                                                                                                  & \textbf{~7 Astor*}~\cite{martinez2016astor}     & -                  & 6/11                 & -                  & -                 & -                 & -                   & 6              \\
                                                                                                  & \textbf{~8 Nopol}~\cite{xuan2017nopol}    & 5/35               & 1/4                  & -                  & -                 & -                 & -                   & 6              \\
                                                                                                  & \textbf{~9 LSRepair}~\cite{liu2018lsrepair}  & 19/37              & -                    & -                  & -                 & -                 & -                   & 19             \\
                                                                                                  & \textbf{10 FixMiner*}~\cite{koyuncu2018fixminer}  & 25/31              & -                    & -                  & -                 & -                 & -                   & 25             \\

\midrule                                                                                                  
                                                                                                  
\multirow{9}{*}[0.5em]{\rotatebox{-90}{\textbf{Supplemented}}}
									 															  & \textbf{11 JAID}~\cite{chen2017contract}      & 9/31               & -                    & -                  & -                 & -                 & -                   & 9              \\
                                                                                                  & \textbf{12 HD-Repair*}~\cite{le2016history} & 13/23              & -                    & -                  & -                 & -                 & -                   & 13             \\
                                                                                                  & \textbf{13 ACS}~\cite{xiong2017precise}      & 18/23              & -                    & -                  & -                 & -                 & -                   & 18             \\
                                                                                                  & \textbf{14 SketchFix*}~\cite{hua2018sketchfix} & 19/26              & -                    & -                  & -                 & -                 & -                   & 19             \\
                                                                                                  & \textbf{15 ssFix*}~\cite{xin2017leveraging}     & 20/60              & -                    & -                  & -                 & -                 & -                   & 20             \\
                                                                                                  & \textbf{16 CapGen*}~\cite{wen2018context}    & 21/25              & -                    & -                  & -                 & -                 & -                   & 21             \\
                                                                                                  & \textbf{17 Elixir*}~\cite{saha2017elixir}    & 26/41              & -                    & -                  & -                 & -                 & -                   & 26             \\
                                                                                                  & \textbf{18 SimFix*}~\cite{jiang2018shaping}    & 34/56              & -                    & -                  & -                 & -                 & -                   & 34             \\
                                                                                                  & \textbf{19 Hercules}~\cite{saha2019harnessing}  & 49/72              & -                    & -                  & -                 & -                 & -                   & 49             \\
                                                                                                  
\midrule                                                                                                  

\multirow{6}{*}[0em]{\rotatebox{-90}{\textbf{Perfect}}}
																								  & \textbf{20 SequenceR}~\cite{liu2018mining}  & 12/19              &   -                    & -                  & -                 & -                 & -                   & 12             \\
                                                                                                  & \textbf{21 kPAR*}~\cite{liu2019you}      & 30/55              & -                    & -                  & -                 & -                 & -                   & 30             \\
                                                                                                  & \textbf{22 AVATAR*}~\cite{liu2019avatar}    & 34/39              & -                    & -                  & -                 & -                 & -                   & 34             \\
                                                                                                  & \textbf{23 TBar}~\cite{Liu:2019:TRT:3293882.3330577}      & \textbf{65/101}             & -                    & -                  & -                 & -                 & -                   & 65             \\
\cmidrule(lr){2-9}
                                                                                                  & \textbf{~~~~\tool}    & \djfix/\djplausible & \textbf{\quixfix / \quixplausible} & \textbf{\codeflawsfix / \codeflawsplausible}   & \cfix$^\dagger$/-      & \textbf{\pythonfix/\pythonplausible}    & \textbf{\jsfix$^\dagger$}/-        & \textbf{\alllanguage}  \\
&      \textbf{(not fixed by others)}                                      & \hilight{\bf (\jsfix)} & \hilight{\bf (\uniquequix)} & \hilight{\textbf{(\uniquecodeflaws)}}   &  \hilight{\textbf{(\uniquemanybugs)}}     & \hilight{\textbf{(\pythonfix)}} &   \hilight{\textbf{(\jsfix)}}      & \hilight{\textbf{(\uniqueall)}}  \\                                                                                                  
\bottomrule
                                                                                                  

\end{tabular}
}
\vspace{-5mm}
\end{table*}




\Comment{

\begin{table*}[t]
\centering
\caption{Comparison with state-of-the-art~\gv approaches. The number of bugs that only ~\tool can fix are in parentheses. The results are displayed as x/y, with x the number of patches semantically equivalent to the developer's patch and y the number of plausible patches. 
\thibaud{I don't really like having a "total" column for everyone, some tools have been used on other datasets we don't use (bugs.jar, introClass, CodRep, etc.}}
\label{tab:comp_trad_approaches}
\adjustbox{max width=0.99\linewidth}{
\begin{tabular}{@{}l|rrrrrrrrrr|rrrrrrrr|rrrrr@{}}
\toprule
        & \multicolumn{10}{c|}{\textbf{Normal FL-based APR}} & \multicolumn{8}{c|}{\textbf{Supplemented FL-based APR}} & \multicolumn{5}{c}{\textbf{Perfect FL-based APR}} \\ 
        \cmidrule{2-24}
\textbf{Datasets}                     & \textbf{GenProg} & \textbf{Kali} & \textbf{Astor} & \textbf{Nopol} & \textbf{FM}      & \textbf{LSRep}       & \textbf{Angelix} & \textbf{RSRep}       & \textbf{Prophet} & \textbf{SPR} & \textbf{Elixir} & \textbf{HERC.} & \textbf{JAID} & \textbf{ssFix}            &\textbf{CG}           & \textbf{SkFix}        & \textbf{ACS}         & \textbf{SimFix}          & \textbf{AVATAR}      & \textbf{kPAR}    & \textbf{TBar}                      & \textbf{SeqR}     &  \textbf{\tool} \\
       
\midrule
\textbf{Defects4J}    & 5/27        & 1/22          & -              & 5/35           & 25/31              & 19/37            & -                & 0/44              & -                & -            & 26/41           &     49/72      & 9/31          & 20/60                   & 21/25                & 19/26                  & 18/23                & 34/56                  &  34/39              &    30*/55        & 65*/101                            &  12/19            & \textbf{\djfix(\uniquedj)/\djplausible }       \\
\addlinespace
\textbf{QuixBugs}     & 0/2         & 1/2           &  6/11          & 1/4            & -                  & -                & -                & 2/4               & -                & -            & -               &  -             & -             & -                       & -                    & -                      & -                    & -                      & -                   & -                & -                                  &  -                &  \textbf{\quixfix(\uniquequix)/\quixplausible}        \\
\midrule
\textbf{Codeflaws}    & -           & -             &     -          & -              & -                  & -                & 317/591          & -                 & -                & -            & -               & -              & -             & -                       & -                    & -                      & -                    & -                      & -                   & -                & -                                  & -                 &  \textbf{\codeflawsfix/ \codeflawsplausible}        \\
\addlinespace
\textbf{ManyBugs}      & 2/18        & 3/27          &     -          & -              & -                  & -                & 18/39            & 2/10              & 15/39            & 11/38        & -               & -              & -             & -                       & -                    & -                      & -                    & -                      & -                   & -                & -                                  & -                 &  \textbf{\cfix/ \cplausible}       \\
\midrule
\textbf{QuixBugs}     & -           & -             & -              & -              & -                  & -                & -                & -                 & -                & -            & -               & -              & -             & -                       & -                    & -                      & -                    & -                      & -                   & -                & -                                  & -                 &  \textbf{\pythonfix/ \pythonplausible}        \\
\midrule
\textbf{JavaScript}   & -           & -             & -              & -              & -                  & -                & -                & -                 & -                & -            & -               & -              & -             & -                       & -                    & -                      & -                    & -                      & -                   & -                & -                                  & -                 &  \textbf{\jsfix/-}       \\
\midrule
\textbf{Total}        & 7           & 5             & 6              & 6              & 25                 & 19               & 335              & 4                 & 15               & 11           & 26              & 49             & 9             & 20                      & 21                   & 19                     & 18                   & 34                     & 34                  & 30               & 65                                 & 12                &  \textbf{\alllanguage}       \\

\bottomrule
\end{tabular}
}
\end{table*}
}


\Comment{
\begin{table*}[t]
\centering
\caption{Comparison with state-of-the-art~\gv approaches. The number of bugs only ~\tool can fix are in parentheses.}
\label{tab:comp_trad_approaches}
\adjustbox{max width=0.99\linewidth}{
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrrr@{}}
\toprule
        & \multicolumn{3}{c}{\textbf{Astor}~\cite{martinez2016astor}}  & \textbf{HDR}    &  \textbf{Nopol}                                & \textbf{ACS}            & \textbf{Elixir}       & \textbf{JAID}           & \textbf{ssFix}           &\textbf{CapGen}        & \textbf{SketchFix}      & \textbf{FixMiner}          & \textbf{LSRepair}      & \textbf{SimFix}         & \textbf{SOFix}       & \textbf{SeqR}       &  \multicolumn{2}{c}{\textbf{\tool}} \\
\cmidrule(rr){2-4}\cmidrule(ll){18-19}
\textbf{Projects}         & \textbf{jGP}        & \textbf{jKali}           & \textbf{jMutR} & \cite{le2016history} & \cite{xuan2017nopol} & \cite{xiong2017precise} & \cite{saha2017elixir} & \cite{chen2017contract} & \cite{xin2017leveraging} & \cite{wen2018context} & \cite{hua2018sketchfix} & \cite{koyuncu2018fixminer} & \cite{liu2018lsrepair} & \cite{jiang2018shaping} & \cite{liu2018mining} & \cite{chen2018sequencer} & Top 1 & All \\

\cmidrule(rr){1-1} \cmidrule(rr){2-4} \cmidrule(rr){5-17} \cmidrule(ll){18-19}

Chart    & 0                        & 0                        & 1                        & 0                    & 1                    & 2                       & 4                     & 2                       & 3                        & 4                     & 6                       & 5                          & 3                      & 4                       & 5                    &  1                       &  2 (0)   &  3 (0)        \\
Closure  & 0                        & 0                        & 0                        & 0                    & 0                    & 0                       & 0                     & 5                       & 2                        & 0                     & 3                       & 5                          & 0                      & 6                       & 0                    &  3                       &  8 (2)   & 11 (5)       \\
Lang     & 0                        & 0                        & 0                        & 2                    & 3                    & 3                       & 8                     & 1                       & 5                        & 5                     & 3                       & 2                          & 8                      & 9                       & 4                    &  2                       &  4 (1)   & 4 (1)         \\
Math     & 5                        & 1                        & 2                        & 4                    & 1                    & 12                      & 12                    & 1                       & 10                       & 12                    & 7                       & 12                         & 7                      & 14                      & 13                   &  5                       &  4 (0)   & 9 (0)         \\
Mockito  & 0                  		 & 0                       & 0                        & 0                    & 0                    & 0                       & 0                     & 0                       & 0                        & 0                     & 0                       & 0                          & 1                      & 0                       & 0                    &  0                       &  0 (0)   & 0 (0)        \\
Time     & 0                        & 0                        & 0                        & 0                    & 0                    & 1                       & 2                     & 0                       & 0                        & 0                     & 0                       & 1                          & 0                      & 1                       & 1                    &  0                       &  1 (0)   & 1 (0)         \\
\cmidrule(rr){1-1} \cmidrule(rr){2-4} \cmidrule(rr){5-17} \cmidrule(ll){18-19}
\textbf{Defects4J}    & 5                        & 1                        & 3                        & 6                    & 5                    & 18                      & 26                    & 9                       & 20                       & 21                    & 19                      & 25                         & 19                     & 34                      & 23                   &  12                      &  \djfirst (3)  & \djfix (6)        \\
\cmidrule(rr){1-1} \cmidrule(rr){2-4} \cmidrule(rr){5-17} \cmidrule(ll){18-19}
\cmidrule(rr){1-1} \cmidrule(rr){2-4} \cmidrule(rr){5-17} \cmidrule(ll){18-19}
     
\textbf{QuixBugs}  &  \multicolumn{3}{c}{6~\cite{Ye2018APRQuixBugs}}                                          & -                                    & 1                                    & -                                   & -                                    & -                                    & -                                      & -                                   & -                                         & -                                           & -                                       & -                                      & -      & -                     &  \quixfirst (10)      &  \quixfix (10)        \\
\bottomrule
\end{tabular}
}
\end{table*}
}


==> tab/coverage_baseline.tex <==
\begin{table}[htbp]
\caption{Branch coverage achieved by libFuzzer and our fuzzer for selective APIs in Tensorflow.}
\label{tab:coverage_baseline}
\begin{center}
\begin{tabular}{lrrr}
\toprule
           & \multicolumn{1}{c}{Covered} & \multicolumn{1}{c}{All} & \multicolumn{1}{c}{Coverage} \\ \hline
libFuzzer  &                              &                          &                               \\ 
\tool &                              &                          &                               \\ \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tab/coverage_constraint.tex <==
\begin{table*}[htbp]
\caption{Branch coverage achieved by with and without constraints of our approach for all available APIs.}
\label{tab:coverage_constraints}
\begin{center}
\begin{tabular}{l|rrr|rrr|rrr}
\toprule
\multirow{2}{*}{} & \multicolumn{3}{c|}{TensorFlow} & \multicolumn{3}{c|}{PyTorch} & \multicolumn{3}{c}{MXNet} \\ \cline{2-10} 
                  & Covered    & All   & Coverage   & Covered   & All  & Coverage  & Covered  & All & Coverage \\ \hline
W/O constraints         &            &       &            &           &      &           &          &     &          \\
\tool        &            &       &            &           &      &           &          &     &         \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> tab/doc_analysis_stat.tex <==
\begin{table}[htbp]
\caption{Documentation Statistics}
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
                                         & \textbf{TensorFlow} & \textbf{PyTorch} & \textbf{MXNet} \\ \midrule
\# words in documentation                 &   527,125           & 144,541           &    364,728       \\
% Documentation  bug              & 15                  & 17               &        22       \\
\# relevent APIs       &   949           & 415           &    959       \\

%Max \# of constraints per API                             & 44                 &     34             &   143             \\
%Avg \# of constraints per API                         & 7.4                &    5.4              &  9.6             \\ 
\bottomrule
\end{tabular}
\label{tab:doc_stat}
\end{table}

==> tab/es_ef_baseline.tex <==
\begin{table}[htbp]
\centering
\caption{Number of bugs found by the baseline and \tool with 50\% $conformRatio$ \yitong{updated ES to be w/o adaptive gen}} \lin{changed ES to CI (conforming inputs), and EF to VI (violating inputs)}
\label{tab:es_ef_baseline}
\begin{tabular}{ll|rrrr}
\toprule
\multicolumn{2}{l|}{\textbf{Approach}} & \multicolumn{1}{l}{\textbf{TensorFlow}} & \multicolumn{1}{l}{\textbf{PyTorch}} & \multicolumn{1}{l}{\textbf{MXNet}} & \multicolumn{1}{l}{\textbf{Total}} \\
\toprule
\multicolumn{2}{l|}{Baseline}          & 14                                      & 5                                    & 1                                  & \baseAll                            \\
\hline
\multirow{3}{*}{\tool}     & CI     & 21                                      & 6                                    & 9                                  & \oursESAll                          \\
                             & VI     & 21                                      & 7                                    & 9                                  & \oursEFAll   \\
      & All    & 25                                      & 11                                   & 10                                 & \oursAll                            \\
\bottomrule
\end{tabular}
\end{table}

==> tab/pattern_example_description.tex <==

\begin{table*}[t]
\centering
\caption{Rule examples and the  extracted constraints from TensorFlow, PyTorch, and MXNet
\todo{}\hung{We need to update the examples here now that we extract the constraints automatically. The extraction rules are now IR mapping in the tree form, not sure how we could display that here without using too much space}
%\lin{from TensorFlow, PyTorch, and MxNet}\danning{added} 
%\lin{do you have a better example for ndim? the current one has optional tensor that distracts readers from the main point. also, it is long. if we have replace it with a shorter one, we can add the variance name to the constraints: n: structure: \{list(int)\}. Do we also extract a dtype tensor from the same sentence? people may have this kind of questions. The same question goes to A string for data\_format. do we extract dtype for that? we will need to explain. it is not a bad idea to show an example where we extract 2-3 constraints from the same line for one parameter. 
%if you want to focus on part of the line, could consider \texttt{weights}: ... whose rank is either 0, and the same rank as \textasciigrave labels\textasciigrave or \texttt{data\_format}: ...  \textasciigrave ``NWC"\textasciigrave~ and \textasciigrave ``NCW"\textasciigrave ~are supported. }\danning{solved, n:structure:\{list(int)\} is weied, especially when it gets several type of constraints. So changed it to ``n:structure=\{list(int)\},shape=\{...\}"}
}
\vspace{-3mm}
\label{tab:pat_example}

\resizebox{\textwidth}{!}{

\begin{tabular}{@{}l@{ }l@{ }l@{\hspace{1mm}}l@{\hspace{1mm}}l@{}}
    \toprule
    
    \textbf{Category}
    &\textbf{No.}
      &\textbf{Examples of extraction rules}
      &\textbf{Examples of sentences from API documents}
      &\textbf{Examples of extracted constraints}
      \\ 
    
    \midrule


    \multirow{2}{*}{\textbf{\datastructure}}
      &1 
      &\textless{}\textit{structure}\textgreater{} (list/tuple/...) of \textless{}\textit{dtype}\textgreater{} &\texttt{n}: A list of integer.
      &\texttt{n}: \texttt{structure=\{list(int)\}}
      \\
      
      &2
      &\textless{}\textit{structure}\textgreater{} (dict/dictionary) of \textless{}\textit{dtype}\textsubscript{1}\textgreater{}~to \textless{}\textit{dtype}\textsubscript{2}\textgreater{}
      &\texttt{features}: Dict of string to \textasciigrave Tensor\textasciigrave.
      &\texttt{features}: \texttt{structure=\{dict(string:tensor)\}}
      \\
    
    \midrule
      
      
         \multirow{3}{*}{\textbf{\dtype}}
      %&must be one of the following types: \textless{}\textit{dtype}\textsubscript{1}\textgreater{}, ...\textless{}\textit{dtype}\textsubscript{n}\textgreater{} &\texttt{input}: Must be one of the following types:\textasciigrave half \textasciigrave,\textasciigrave float32\textasciigrave, \textasciigrave float64\textasciigrave.  
      %&\texttt{input}: \texttt{dtype=\{float16, float32, float64\}} dtype:\{\texttt{float16}, \texttt{float32}, \texttt{float64} \} 
      %\\
    &3
      &of/with type \textless{}\textit{dtype}\textgreater{} 
      &\texttt{audio}: A \textasciigrave~Tensor\textasciigrave~of type \textasciigrave~float32\textasciigrave.
      &\texttt{input}: \texttt{dtype=\{float32\}},\texttt{structure=\{tensor\}}
      \\
    &4
      &\textless{}\textit{ndim}\textgreater{}-d/dimensional \textless{}\textit{dtype}\textgreater~tensor &\texttt{mask}: K-D boolean tensor. 
      &\texttt{mask}: \texttt{dtype=\{boolean\},ndim=\{k\}},\texttt{structure=\{tensor\}}  \\ 
      
      &5
      &must have the same type/dtype as \textless{}\textit{dependency}\textgreater &\texttt{imag}: Must have the same type as \textasciigrave real\textasciigrave.
      &\texttt{imag}: \texttt{dtype=\{\&real.dtype\}}  
      \\  
    
    \midrule
     
      %&whose rank is either \textless{}\textit{ndim}\textgreater{}, or the same rank as \textless{}\textit{dependency}\textgreater{} 
      %&\texttt{weights}: Optional \textasciigrave Tensor\textasciigrave ~whose rank is either 0, or the same rank as \textasciigrave labels\textasciigrave.
      %&\texttt{ndim:\{0,\&labels.ndim}\}
      %\\
    
    \multirow{4}{*}{\textbf{\shape}} 
    &6
      &\textless{}\textit{ndim}\textgreater{}-d/dimension tensor & \texttt{logits}: 2-D Tensor..
      &\texttt{logits}: \texttt{ndim=\{2}\},\texttt{structure=\{tensor}\}
      \\ 
      &7
      &with/of the same shape as  \textless{}\textit{dependency}\textgreater{}, 
      &\texttt{target}: A tensor with the same shape as \textasciigrave output\textasciigrave.
      &\texttt{target}: \texttt{shape=\{\&output.shape}\}
      \\
      
      &8
      &of/with shape \textless{}\textit{shape}\textgreater{} 
      &\texttt{weights}: ...of shape \textasciigrave[num\_classes, dim]\textasciigrave.
      &\texttt{weights}: \texttt{shape=\{[\&num\_classes,dim]\}}
      \\
      &9
      &tensor of length \textless{}\textit{shape}\textgreater{}
      &\texttt{rates}: A 1-D Tensor of length 4.
      &\texttt{rates}: \texttt{shape=\{[4]}\}
      \\
    
    \midrule
      
    \multirow{3}{*}{\textbf{\validvalue}}
    &10
      &only \textless{}\textit{value}\textsubscript{1}\textgreater{}, ... \textless{}\textit{value}\textsubscript{n}\textgreater{} are supported & \texttt{data\_format}: A string. Only \textasciigrave ``NWC"\textasciigrave~ and \textasciigrave ``NCW"\textasciigrave ~are supported. 
      &\texttt{data\_format}: \texttt{dtype=\{string\}},\texttt{enum=\{"NWC","NCW"\}}
      \\
      
      &11
      & non-negative \textless{}\textit{dtype}\textgreater{} 
      & \texttt{num\_columns}: ... non-negative integer... 
      &\texttt{num\_columns}:\texttt{range=\{[0,inf)\},dtype:\{int\}}
      \\
      
      &12
      & must be in the range \textless{}\textit{valid range}\textgreater{}.
      & \texttt{axis}: Must be in the range \textasciigrave[-rank(input), rank(input))\textasciigrave
      &\texttt{axis}: \texttt{range=\{[-\&input.ndim,\&input.ndim)\}}
      \\ 
    
    \bottomrule
  
\end{tabular}
}
\vspace{-3mm}
\end{table*}





% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \caption{Example of Patterns}
% \label{tab:pat_example}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllll@{}}
% \toprule
% \textbf{Constraint Category}                   & \textbf{Example Rules} & \multicolumn{2}{l}{\textbf{Example from Documents}} & \textbf{Constraints Extracted} \\
%                                               &                        & \textbf{Parameter}        & \textbf{Sentence}       &                                \\ \midrule
% \multirow{2}{*}{\dtype} &
%   must be one of the following types: \textless{}\dtype\textsubscript{1}\textgreater{}, ...\textless{}\dtype\textsubscript{n}\textgreater{} &
%   \texttt{input} &
%   Must be one of the following types:\textasciigrave half \textasciigrave,\textasciigrave float32\textasciigrave, \textasciigrave float64\textasciigrave.  &
%   \dtype:\{\texttt{float16}, \texttt{float32}, \texttt{float64} \} \\
%                                               &      \textless{}\shape\textgreater{}-d/dimensional \textless{}\dtype \textgreater~tensor & \texttt{mask}&
%   K-D boolean tensor &
%   \dtype:\{\texttt{boolean}\}  
                                               
%                                               \\ \midrule
                                               
                                               
% \multirow{2}{*}{\datastructure} &   \textless{}\datastructure\textgreater{} (list/tuple/...) of \textless{}\dtype\textgreater{} &\texttt{n}&
%   A list of integer. &
%   \texttt{list(int)} 

% \\
% &        \textless{}\datastructure\textgreater{} (dict/dictionary) of \textless{}\dtype\textsubscript{1}\textgreater{}~to \textless{}\dtype\textsubscript{2}\textgreater{} & \texttt{features}&
%   dict of string to \textasciigrave Tensor\textasciigrave. &
%   \texttt{dict(string:tensor)} 
% \\ \midrule


% \multirow{2}{*}{\shape}         &  of/with shape \textless{}\shape\textgreater{} & \texttt{x1}&
%   input tensor of shape B  times P  times M. &
%   \texttt{shape:{[}b, p, m{]}}                             \\
%                                               & 
%                                               whose rank is either \textless{}\shape\textgreater{}, or the same rank as \textless{}\textit{dependency}\textgreater{} & \texttt{weights}&
%   Optional \textasciigrave Tensor\textasciigrave ~whose rank is either 0, or the same rank as \textasciigrave labels\textasciigrave &
%   \texttt{ndim:\{0,\&labels}\}\\
%                                               \midrule
                                               
                                               
% \multirow{2}{*}{\validvalue}   &   only \textless{}\textit{value}\textsubscript{1}\textgreater{}, ... \textless{}\textit{value}\textsubscript{n}\textgreater{} are supported & \texttt{data\_format} &
%   A string. \textasciigrave ``NWC"\textasciigrave~ and \textasciigrave ``NCW"\textasciigrave ~are supported. &
%   \texttt{enum:\{"NWC","NCW"\}}                               \\
%                                               & must be in the range \textless{}\textit{valid range}\textgreater{} & \texttt{axis}&
%   Must be in the range \textasciigrave{[}-rank(input), rank(input))\textasciigrave &
%   \texttt{range:{[}-\&input.ndim,\&input.ndim)}                               \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

==> tab/ratio_analysis.tex <==
\begin{table}[htbp]
\caption{Bug detection sensitivity analysis for the ratio of Expecting Success (ES) and Expecting Failure (EF). \yitong{to be removed}}
\label{tab:ratio_analysis}
\begin{tabular}{c|rrr|rrr|rrr}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}ES vs EF \\ \%\end{tabular}}}} & \multicolumn{3}{c|}{\textbf{TensorFlow}}                                   & \multicolumn{3}{c|}{\textbf{PyTorch}}                                      & \multicolumn{3}{c}{\textbf{MXNet}}                                        \\ \cline{2-10} 
\multicolumn{1}{c|}{}                                                                                 & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c|}{All} & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c|}{All} & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c}{All} \\
\midrule
0 vs 100                                                                                              & 0                      & 22                     & 22                       & 0                      & 8                      & 8                        & 0                      & 9                      & 9                        \\
10 vs 90                                                                                              & 17                     & 22                     & 23                       & 5                      & 8                      & 10                       & 4                      & 9                      & 9                        \\
20 vs 80                                                                                              & 18                     & 22                     & 23                       & 6                      & 8                      & 11                       & 6                      & 9                      & 10                       \\
30 vs 70                                                                                              & 20                     & 21                     & 24                       & 7                      & 8                      & 12                       & 7                      & 9                      & 10                       \\
40 vs 60                                                                                              & 20                     & 21                     & 24                       & 7                      & 7                      & 11                       & 7                      & 9                      & 10                       \\
50 vs 50                                                                                              & 20                     & 21                     & 24                       & 7                      & 7                      & 11                       & 8                      & 9                      & 10                       \\
60 vs 40                                                                                              & 20                     & 21                     & 24                       & 8                      & 6                      & 11                       & 8                      & 9                      & 10                       \\
70 vs 30                                                                                              & 20                     & 20                     & 24                       & 8                      & 6                      & 11                       & 8                      & 8                      & 10                       \\
80 vs 20                                                                                              & 20                     & 20                     & 24                       & 8                      & 6                      & 11                       & 8                      & 8                      & 10                       \\
90 vs 10                                                                                              & 20                     & 17                     & 24                       & 9                      & 3                      & 11                       & 8                      & 6                      & 10                       \\
100 vs 0                                                                                              & 21                     & 0                      & 21                       & 10                     & 0                      & 10                       & 8                      & 0                      & 8                       \\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
\centering
\begin{tabular}{l|rrr|rrr|rrr|rrr}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}ES vs EF \\ \%\end{tabular}}}} & \multicolumn{3}{c|}{\textbf{TensorFlow}}                                   & \multicolumn{3}{c|}{\textbf{PyTorch}}                                      & \multicolumn{3}{c|}{\textbf{MXNet}}                                        & \multicolumn{3}{c}{\textbf{Total}}                                        \\ \cline{2-13} 
\multicolumn{1}{c|}{}                                                                                 & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c|}{All} & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c|}{All} & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c|}{All} & \multicolumn{1}{c}{ES} & \multicolumn{1}{c}{EF} & \multicolumn{1}{c}{All} \\
\midrule
0 vs 100                        & 0                      & 22                     & 22                        & 0                      & 8                      & 8                         & 0                      & 9                      & 9                         & 0                      & 39                     & 39                        \\
10 vs 90                        & 17                     & 22                     & 23                        & 5                      & 8                      & 10                        & 4                      & 9                      & 9                         & 26                     & 39                     & 65                        \\
20 vs 80                        & 18                     & 22                     & 23                        & 6                      & 8                      & 11                        & 6                      & 9                      & 10                        & 30                     & 39                     & 69                        \\
30 vs 70                        & 20                     & 21                     & 24                        & 7                      & 8                      & 12                        & 7                      & 9                      & 10                        & 34                     & 38                     & 72                        \\
40 vs 60                        & 20                     & 21                     & 24                        & 7                      & 7                      & 11                        & 7                      & 9                      & 10                        & 34                     & 37                     & 71                        \\
50 vs 50                        & 20                     & 21                     & 24                        & 7                      & 7                      & 11                        & 8                      & 9                      & 10                        & 35                     & 37                     & 72                        \\
60 vs 40                        & 20                     & 21                     & 24                        & 8                      & 6                      & 11                        & 8                      & 9                      & 10                        & 36                     & 36                     & 72                        \\
70 vs 30                        & 20                     & 20                     & 24                        & 8                      & 6                      & 11                        & 8                      & 8                      & 10                        & 36                     & 34                     & 70                        \\
80 vs 20                        & 20                     & 20                     & 24                        & 8                      & 6                      & 11                        & 8                      & 8                      & 10                        & 36                     & 34                     & 70                        \\
90 vs 10                        & 20                     & 17                     & 24                        & 9                      & 3                      & 11                        & 8                      & 6                      & 10                        & 37                     & 26                     & 63                        \\
100 vs 0                        & 21                     & 0                      & 21                        & 10                     & 0                      & 10                        & 8                      & 0                      & 8                         & 39                     & 0                      & 39             \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}
